Portable Multi-Hypothesis Monte Carlo Localization for Mobile Robots

Self-localization is a fundamental capability that mobile robot navigation systems integrate to move from one point to another using a map. Thus, any enhancement in localization accuracy is crucial to perform delicate dexterity tasks. This paper describes a new location that maintains several populations of particles using the Monte Carlo Localization (MCL) algorithm, always choosing the best one as the sytems's output. As novelties, our work includes a multi-scale match matching algorithm to create new MCL populations and a metric to determine the most reliable. It also contributes the state-of-the-art implementations, enhancing recovery times from erroneous estimates or unknown initial positions. The proposed method is evaluated in ROS2 in a module fully integrated with Nav2 and compared with the current state-of-the-art Adaptive ACML solution, obtaining good accuracy and recovery times.

==> Old/Intro_alternative.tex <==

The fundamental capability of a mobile robot is navigation. Navigation allows a robot to use a map to locate itself, plan routes from origin to destination, and carry them out. Even though navigation has been working for decades, the problem is still far from being solved. One of the main issues is reproducibility: on the one hand,  it is hard finding robust algorithms that can be applied in a general way to different robots and scenarios.
On the other hand, finding localization algorithms in public repositories correctly implemented and  easy to replicate it is not an easy task. Thus, it is not surprising that many works have not survived the robot for which they were designed, the laboratory in which they were implemented, or the paper in which they were presented. 

To solve first limitation, this research proposes a localization method that allows AMCL to become a global approximation, capable of recovering from a situation of total ignorance, common at startup, and maintaining other hypotheses, useful in case of loss or hijacking. Our approach maintains several AMCLs, each of them independent. The novel contributions of this aproach are:

\begin{enumerate}
    \item A metric to determine if an AMCL is wrong. Usually, the uncertainty derived from the AMCL covariance matrix is used to determine when the estimate has deteriorated. This is ineffective since this deterioration could be due to many other causes than a wrong estimate. Also, estimates with low uncertainty could be completely wrong. Our metric directly measures the consistency between the sensory measurements obtained with those expected for each particle of each AMCL. We will demonstrate how this metric allows you to compare two AMCLs effectively.
    \item An observation model based on geometric transformations and projections in this work is limited in contrast to a 2D map but perfectly supports 3D maps and sensors.
    \item A dynamics of the collection of AMCLs. We will show how our approach can maintain different AMCLs, created in positions consistent with the observations and continuously evaluated to eliminate erroneous ones or merge them with each other if they converge to similar positions.  
    \item A system and methodology used in the validation. We have developed a series of components within the MOCAP4ROS2 framework, which allows us to use a motion capture system fully integrated with ROS2 to measure the metrics that determine whether a localization method improves an existing one.
\end{enumerate}


Second limitation is faced by the Open Source development model. It  has brought many benefits to industry in general and to science in particular. Analyzing and executing publicly available implementations favors one of the principles of the scientific method: the reproducibility of scientific studies. In Robotics, ROS~\cite{quigley2009ros}, and the current version, ROS2~\cite{doi:10.1126/scirobotics.abm6074}, have greatly facilitated the reuse of other scientists' implementations by becoming the \emph{de facto} standard in robot software development, supporting hundreds of robots of different configurations and manufacturers. Nav2  \cite{macenski2020marathon2} is their navigation framework, which aspires to be the world's most widely used navigation system. The implementation of the work presented in this paper has been integrated into Nav2 so that it can be reused by other robotics researchers, guaranteeing that our method is general and applicable to any robot using Nav2.



This paper is organized as follows: After presenting the works most related works to ours in section \ref{sec:related}, in section \ref{sec:amcl} we will show the mathematical foundations of the AMCL used, emphasizing contribution 2. Section \ref{sec:mhamcl} brings together contributions 1 and 3, and presents how different AMCLs are maintained. The experimental validation, including contribution 4, is presented in section \ref{sec:validation}.



% The fundamental capability of a mobile robot is navigation. Navigation allows a robot to use a map to locate itself, plan routes from origin to destination, and carry them out. Even though navigation has been working for decades, the problem is still far from being solved. One of the main issues is reproducibility: on the one hand,  it is hard finding robust algorithms that can be applied in a general way to different robots and scenarios.
% On the other hand, finding localization algorithms in public repositories correctly implemented and  easy to replicate it is not an easy task. Thus, it is not surprising that many works have not survived the robot for which they were designed, the laboratory in which they were implemented, or the paper in which they were presented. 

% In recent times, the Open Source development model has brought many benefits to industry in general and to science in particular. Analyzing and executing publicly available implementations favors one of the principles of the scientific method: the reproducibility of scientific studies. In Robotics, ROS~\cite{quigley2009ros}, and the current version, ROS2~\cite{doi:10.1126/scirobotics.abm6074}, have greatly facilitated the reuse of other scientists' implementations by becoming the \emph{de facto} standard in robot software development, supporting hundreds of robots of different configurations and manufacturers. Nav2  \cite{macenski2020marathon2} is their navigation framework, which aspires to be the world's most widely used navigation system. The implementation of the work presented in this paper has been integrated into Nav2 so that it can be reused by other robotics researchers, guaranteeing that our method is general and applicable to any robot using Nav2.

% Localization in Mobile Robotics is a robot's ability to know its position on a map. Navigating from one coordinate to another in the environment needs localization since the routes generated are coded as map coordinates. There are global and local location approaches. The global approaches allow to locate a robot from total ignorance and maintain the possible positions of the robot within the map. These methods are usually based on a grid~\cite{buschka2000fuzzy}, where each cell, divided in orientations, codes the probability of the robot's presence. Local approximations, or tracking, start from a known position and try to correct errors in the displacement (or in its perception) to calculate the position as precisely as possible. The Extended Kalman Filter~\cite{teslic2011ekf} (EKF) is the most representative tracking location method. The Monte Carlo method~\cite{dellaert1999monte}(MCL), also called Particle Filter, is considered state of the art in robot location due to its flexibility and precision. As a sampled probability distribution of the robot's position, it is a local location method, so the robot's position must be known a priori, and it can only maintain one hypothesis. Some approximations allow some degree of relocation~\cite{lenser2000sensor}, giving the appearance of a global method. Still, recovering when it converges to a position if the estimate is wrong it is difficult.

% To solve this limitation, we have developed a localization method that allows AMCL to become a global approximation, capable of recovering from a situation of total ignorance, common at startup, and maintaining other hypotheses, useful in case of loss or hijacking. Our approach maintains several AMCLs, each of them independent. The novel contributions of this work are:

% \begin{enumerate}
%     \item A metric to determine if an AMCL is wrong. Usually, the uncertainty derived from the AMCL covariance matrix is used to determine when the estimate has deteriorated. This is ineffective since this deterioration could be due to many other causes than a wrong estimate. Also, estimates with low uncertainty could be completely wrong. Our metric directly measures the consistency between the sensory measurements obtained with those expected for each particle of each AMCL. We will demonstrate how this metric allows you to compare two AMCLs effectively.
%     \item An observation model based on geometric transformations and projections in this work is limited in contrast to a 2D map but perfectly supports 3D maps and sensors.
%     \item A dynamics of the collection of AMCLs. We will show how our approach can maintain different AMCLs, created in positions consistent with the observations and continuously evaluated to eliminate erroneous ones or merge them with each other if they converge to similar positions.  
%     \item A system and methodology used in the validation. We have developed a series of components within the MOCAP4ROS2 framework, which allows us to use a motion capture system fully integrated with ROS2 to measure the metrics that determine whether a localization method improves an existing one.
% \end{enumerate}

% This paper is organized as follows: After presenting the works most related works to ours in section \ref{sec:related}, in section \ref{sec:amcl} we will show the mathematical foundations of the AMCL used, emphasizing contribution 2. Section \ref{sec:mhamcl} brings together contributions 1 and 3, and presents how different AMCLs are maintained. The experimental validation, including contribution 4, is presented in section \ref{sec:validation}.

==> Old/Intro_original.tex <==
The fundamental capability of a mobile robot is navigation. Navigation allows a robot to use a map to locate itself, plan routes from origin to destination, and carry them out. Even though navigation has been working for decades, the problem is still far from being solved. The fundamental problem is finding robust algorithms that can be applied in a general way to different robots and scenarios that are still efficient.
It is not surprising that many works have not survived the robot for which they were designed, the laboratory in which they were implemented, or the paper in which they were presented. 

In recent times, the Open Source development model has brought many benefits to industry in general and to science in particular. Analyzing and executing publicly available implementations favors one of the principles of the scientific method: the reproducibility of scientific studies. In Robotics, ROS~\cite{quigley2009ros}, and the current version, ROS2~\cite{doi:10.1126/scirobotics.abm6074}, have greatly facilitated the reuse of other scientists' implementations by becoming the \emph{de facto} standard in robot software development, supporting hundreds of robots of different configurations and manufacturers. Nav2  \cite{macenski2020marathon2} is their navigation framework, which aspires to be the world's most widely used navigation system. The implementation of the work presented in this paper has been integrated into Nav2 so that it can be reused by other robotics researchers, guaranteeing that our method is general and applicable to any robot using Nav2.

Localization in Mobile Robotics is a robot's ability to know its position on a map. Navigating from one coordinate to another in the environment needs localization since the routes generated are coded as map coordinates. There are global and local location approaches. The global approaches allow to locate a robot from total ignorance and maintain the possible positions of the robot within the map. These methods are usually based on a grid~\cite{buschka2000fuzzy}, where each cell, divided in orientations, codes the probability of the robot's presence. Local approximations, or tracking, start from a known position and try to correct errors in the displacement (or in its perception) to calculate the position as precisely as possible. The Extended Kalman Filter~\cite{teslic2011ekf} (EKF) is the most representative tracking location method. The Monte Carlo method~\cite{dellaert1999monte}(MCL), also called Particle Filter, is considered state of the art in robot location due to its flexibility and precision. As a sampled probability distribution of the robot's position, it is a local location method, so the robot's position must be known a priori, and it can only maintain one hypothesis. Some approximations allow some degree of relocation~\cite{lenser2000sensor}, giving the appearance of a global method. Still, recovering when it converges to a position if the estimate is wrong it is difficult.

To solve this limitation, we have developed a localization method that allows AMCL to become a global approximation, capable of recovering from a situation of total ignorance, common at startup, and maintaining other hypotheses, useful in case of loss or hijacking. Our approach maintains several AMCLs, each of them independent. The novel contributions of this work are:

\begin{enumerate}
    \item A metric to determine if an AMCL is wrong. Usually, the uncertainty derived from the AMCL covariance matrix is used to determine when the estimate has deteriorated. This is ineffective since this deterioration could be due to many other causes than a wrong estimate. Also, estimates with low uncertainty could be completely wrong. Our metric directly measures the consistency between the sensory measurements obtained with those expected for each particle of each AMCL. We will demonstrate how this metric allows you to compare two AMCLs effectively.
    \item An observation model based on geometric transformations and projections in this work is limited in contrast to a 2D map but perfectly supports 3D maps and sensors.
    \item A dynamics of the collection of AMCLs. We will show how our approach can maintain different AMCLs, created in positions consistent with the observations and continuously evaluated to eliminate erroneous ones or merge them with each other if they converge to similar positions.  
    \item A system and methodology used in the validation. We have developed a series of components within the MOCAP4ROS2 framework, which allows us to use a motion capture system fully integrated with ROS2 to measure the metrics that determine whether a localization method improves an existing one.
\end{enumerate}

This paper is organized as follows: After presenting the works most related works to ours in section \ref{sec:related}, in section \ref{sec:amcl} we will show the mathematical foundations of the AMCL used, emphasizing contribution 2. Section \ref{sec:mhamcl} brings together contributions 1 and 3, and presents how different AMCLs are maintained. The experimental validation, including contribution 4, is presented in section \ref{sec:validation}.
